Deep Nonparametric Convexified Filtering for Computational Photography, Image Synthesis and Adversarial Defense

We aim to provide a general framework of for computational photography that recovers the real scene from imperfect images, via the Deep Nonparametric Convexified Filtering (DNCF). It is consists of a nonparametric deep network to resemble the physical equations behind the image formation, such as denoising, super-resolution, inpainting, and flash. DNCF has no parameterization dependent on training data, therefore has a strong generalization and robustness to adversarial image manipulation. During inference, we also encourage the network parameters to be nonnegative and create a bi-convex function on the input and parameters, and this adapts to second-order optimization algorithms with insufficient running time, having 10X acceleration over Deep Image Prior. With these tools, we empirically verify its capability to defend image classification deep networks against adversary attack algorithms in real-time.

==> figures/ddip_dehaze.tex <==
\begin{figure*}[htbp]
	%	\vspace{-10pt}
	\centering
	\subfigure [Original image]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.46\textwidth]{figures/dehaze_exp/hongkong_0_original.jpg}}
% 	\subfigure [Target image in RD$0$]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/hongkong_0_final.jpg}}
% 	\subfigure [transmission map in RD$1$]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/hongkong_rd1_t.jpg}}
% 	\subfigure [Target image in RD$1$]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/hongkong_rd1_final.jpg}}
 	\subfigure [DIP in RD$1$]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.46\textwidth]{figures/dehaze_exp/hongkong_rd1_final.jpg}}
	\subfigure [CDIP in RD$1$]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.46\textwidth]{figures/dehaze_exp/hongkong_rd1_dcvx_3e-05_final.jpg}}
	\subfigure [DIP in RD$2$]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.46\textwidth]{figures/dehaze_exp/hongkong_rd2_final.jpg}}
	%	\subfigure [input convex neural network (all weights being nonnegative).]% [Loss functions by multi-thread atomically updating SVM.]
	%	{\includegraphics[width=0.5\textwidth]{figures/icnn_nc32}}
% 	\vspace{-10pt}
%	\caption{ Dehazing for the image \textit{HongKong}. %(Including above and below figures)
% 	}
% 	\label{fig:dehaze1}
% 	\vspace{-10pt}
% \end{figure*}
% \begin{figure*}[htbp]
% 		%\vspace{-10pt}
% 	\centering
	\subfigure [Original image]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_0_original.jpg}}
% 	\subfigure [Target image in RD$0$]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_0_final.jpg}}
% 	\subfigure [transmission map in RD$1$]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_rd1_t.jpg}}
% 	\subfigure [Target image in RD$1$]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_rd1_final.jpg}}
	\subfigure [DIP  in RD$0$]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_0_final.jpg}}
	\subfigure [CDIP  in RD$0$]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_0_dcvx_3e-05_final.jpg}}
	\subfigure [DIP  in RD$1$]% [Loss functions by multi-thread atomically updating SVM.]
	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_0_final.jpg}}
% 	\subfigure [DIP  in RD$2$]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.23\textwidth]{figures/dehaze_exp/tiananmen_rd2_final.jpg}}
	%	\subfigure [input convex neural network (all weights being nonnegative).]% [Loss functions by multi-thread atomically updating SVM.]
	%	{\includegraphics[width=0.5\textwidth]{figures/icnn_nc32}}
	\vspace{-10pt}
	\caption{ Visualization of image dehazing. $RD \#0$ denotes the results from $0$th round, where each round has $2000$ iterations. CDIP achieves comparable result to DIP using less than one round. %(Including above and below figures)
	}
	\label{fig:dehaze}
	\vspace{-10pt}
\end{figure*}



==> figures/dip_exp2.tex <==


% \begin{figure*}[htbp]
% 		%\vspace{-10pt}
% 	\centering
% 	\subfigure [Flash image ]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.235\textwidth]{figures/flash/original_f.png}}
% 	\subfigure [No-Flash image]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.235\textwidth]{figures/flash/original_nf.png}}
% 	\subfigure [Imaging with  DIP]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.235\textwidth]{figures/flash/antique_iter350.png}}
% 	\subfigure [Imaging with  CDIP]% [Loss functions by multi-thread atomically updating SVM.]
% 	{\includegraphics[width=0.235\textwidth]{figures/flash/antique_dcvx_iter350.png}}
% 	\vspace{-10pt}
% 	\caption{ Visualization of Flash-no flash imaging. %(Including above and below figures)
% 	}
% 	\label{fig:flash}
% 	\vspace{-10pt}
% \end{figure*}



==> figures/name.tex <==
\begin{figure}[htbp]\label{fig:flash_outlist}
% \subfigure [Convergence of optimization.]% procedure with both convexification and decomposition (DCVX-DIP).]% [Loss functions by 
% 		{\includegraphics[width=0.34\textwidth]{figures/flash/dcvx_converge.png}}
	\subfigure %[In left-right, top-down order, flash image, initialized $I_t$, $5$ middle results by every 200 iterations, last one is the original non-flash image. ]% [Loss functions by 
		{\includegraphics[width=0.5\textwidth]{figures/cw_attack.eps}}
	%\vspace{-10pt}
	%\caption{ Visualization of the optimization procedure. In left-right, top-down order, flash image, initialized $I_t$, $5$ middle results by every 200 iterations, and then the original non-flash image. }
	%\label{fig:icnn}
	\vspace{-10pt}
\end{figure}
